How Does a Neural Network's Architecture Impact Its Robustness to Noisy Labels?

Noisy labels are inevitable in large real-world datasets. In this work, we explore an area understudied by previous works -- how the network's architecture impacts its robustness to noisy labels. We provide a formal framework connecting the robustness of a network to the alignments between its architecture and target/noise functions. Our framework measures a network's robustness via the predictive power in its representations -- the test performance of a linear model trained on the learned representations using a small set of clean labels. We hypothesize that a network is more robust to noisy labels if its architecture is more aligned with the target function than the noise. To support our hypothesis, we provide both theoretical and empirical evidence across various neural network architectures and different domains. We also find that when the network is well-aligned with the target function, its predictive power in representations could improve upon state-of-the-art (SOTA) noisy-label-training methods in terms of test accuracy and even outperform sophisticated methods that use clean labels.

==> fig_GNN_embed.tex <==
\begin{figure*}[h]
     \centering
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{GNN_max_sum_gaussian_mean10_reg_true_label.pdf}
         \caption{Representations colored with true labels}
         \label{fig:maxdeg-clean}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{GNN_max_sum_gaussian_mean10_reg_noisy_label.pdf}
         \caption{Representations colored with noisy labels}
         \label{fig:maxdeg-noisy}
     \end{subfigure}
     \caption{\textbf{PCA visualization of hidden representations} for a GNN trained under noisy labels. 
     We plot the learned representations before the final MLP using training data.
     The task is to predict the maximum degree of the graph, and we use max-sum GNN, an architecture suited for this task.
     Examples are colored with true labels (left) or noisy labels (right).
     The representations have a clear linear relationship with the true labels (left). 
     However, the model cannot recover this relationship because of the noisy labels (right), leading to a large test error. 
     All training labels are corrupted by adding a Gaussian noise drawn from $\mathcal{N}(10,\,15)$.
     }
     \label{fig:maxdeg_graph_embed}
\end{figure*}

==> gnn_structure_compare.tex <==
\begin{table}[t]
    \small
    \begin{center}
    \begin{tabular}{c |c c c }
        \toprule
        %Architecture
        & DeepSet & max-max GNN & max-sum GNN \\
        \midrule
        Use neighborhood information & \xmark & \cmark & \cmark \\
        \begin{tabular}{@{}c@{}} Good at learning signal \end{tabular}  & \cmark & \cmark & \xmark \\
        \begin{tabular}{@{}c@{}} Good at learning noise \end{tabular}  & \xmark & \xmark & \cmark \\
        \bottomrule
    \end{tabular}
    \end{center}
    \vspace{-1em}
    \caption{\textbf{Summary of various GNNs' abilities to learn the signal (max node feature) and the noise (max degree of the graph).} 
    These three properties demonstrate a) DeepSet is good at learning the signal and incapable of learning the noise; b) max-max GNN is better at learning the signal than the noise; c) instead, max-sum GNN is better at learning the noise than the signal.
    The results follow from~\cite{Xu2020What}.}
    \label{table:gnn_structured_noise_compare}
\end{table}
